A New Lower Bound for Agnostic Learning with Sample Compression Schemes

We establish a tight characterization of the worst-case rates for the excess risk of agnostic learning with sample compression schemes and for uniform convergence for agnostic sample compression schemes. In particular, we find that the optimal rates of convergence for size-$k$ agnostic sample compression schemes are of the form $\sqrt{\frac{k \log(n/k)}{n}}$, which contrasts with agnostic learning with classes of VC dimension $k$, where the optimal rates are of the form $\sqrt{\frac{k}{n}}$.

==> intro.tex <==
\section{Introduction}

Compression-based arguments provide some of the simplest and tightest generalization bounds in the literature.
These are
known as {\em Occam learning} in the most general setting
\citep{MR1072253},
and
the special case of {\em sample compression}
\citet{warmuth86,MR1383093,DBLP:journals/ml/GraepelHS05,DBLP:journals/ml/FloydW95}
has been receiving a fair amount of recent attention
\citep{DBLP:journals/jacm/MoranY16,david2016supervised,DBLP:conf/colt/Zhivotovskiy17,hks18}.

As the present paper deals with lower bounds, we stress up-front that
these are {\em statistical} lower bounds (rather than, say, computational \citep{DBLP:conf/nips/GottliebKN14}
or 
communication-based
\citep{DBLP:journals/corr/abs-1711-05893}).
%We shall follow the presentation and terminology of
%\citet{DBLP:journals/ml/GraepelHS05},
%whose Theorem 1 states that 
In the realizable case, \citet{warmuth86,DBLP:journals/ml/FloydW95} 
showed that a $k$-compression scheme
on a sample of size $n \geq e k$
achieves an expected generalization error bound of order
\beqn
\label{eq:realizable-compress}
\frac{ k \log( n / k ) }{n}
%\frac1{n-k}\paren{
%  (k+1)\log n+\log(1/\delta)}.
\eeqn
As the compression size $k$ is a rough analogue of the VC-dimension, one is immediately led to
inquire into the necessity of the $\log (n/k)$ factor. While known to be removable
from the realizable VC bound
\citep{DBLP:journals/iandc/HausslerLW94,DBLP:journals/jmlr/Hanneke16},
the $\log (n/k)$ factor in (\ref{eq:realizable-compress}) turns out to be tight
\citep{DBLP:journals/ml/FloydW95}.
On the other hand, turning to the agnostic case, 
%here 
the corresponding compression result from 
%\citet[Theorem 2]{DBLP:journals/ml/GraepelHS05}
\citet{DBLP:journals/ml/GraepelHS05}
implies an upper bound on the expected excess generalization error
of a certain $k$-compression scheme %(based on empirical risk minimization) 
on a sample of size $n \geq e k$ by a bound of order 
\beqn
\label{eq:agnostic-compress}
\sqrt{\frac{k \log(n/k)}{n}}.
%\frac{n}{n-k}\hat\epsilon
%+
%\sqrt{\frac{
%    (k+2)\log n+\log(1/\delta)}{2(n-k)}}.
\eeqn
Here again, the agnostic VC analogue of (\ref{eq:agnostic-compress})
\citep[Theorem 4.10]{MR1741038}
%**give reference**
might suggest that the $\log (n/k)$ factor might be superfluous.
Though it is a simpler matter to give an $\Omega(\sqrt{k/n})$
lower bound, % nearly matching (\ref{eq:agnostic-compress})\footnote{
%  We were not able to locate such a bound in the literature.
%}, 
it proves significantly more challenging to determine whether the factor of $\log(n/k)$ 
is required for this general bound.  As our main result in this work (Section~\ref{sec:order-indep}), we prove that 
this $\log(n/k)$ factor in (\ref{eq:agnostic-compress}) \emph{cannot} be removed.
%Specifically, we construct a reconstruction function such that, for all compression functions, 
%a lower bound of the form \eqref{eq:agnostic-compress} holds.  
We also prove an analogous 
lower bound for order-dependent compression schemes (Section~\ref{sec:order-dep}),
where the factor becomes $\log(n)$, 
which again is tight.
%again matching a known upper bound.

\hide{
cite floyd+warmth,
our recent compression paper,
thank Nikita
}


==> mycommon.tex <==
\usepackage{mysymbols}
%\usepackage{../latex_files/mytheo}
\usepackage{mathrsfs}
\usepackage{amssymb}
\usepackage{latexsym}
\usepackage{amsmath,amsthm}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{soul}
\usepackage{url}
\usepackage{accents}
%\usepackage{array,multirow}

\newcommand{\pstar}{\mbox{(*)}}
\newcommand{\psstar}{\mbox{(**)}}
\newcommand{\pssstar}{\mbox{(***)}}

\usepackage{stmaryrd}
\DeclareMathOperator*{\bigtimes}{\vartimes}

%\renewcommand{\vec}[1]{\ensuremath{\text{{\bf\textrm{#1}}}}}
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\supp}{\operatorname{supp}}
%\newcommand{\cone}{\operatorname{cone}}
\newcommand{\core}{\operatorname{core}}
\newcommand{\epi}{\operatorname{epi}}
%\renewcommand{\span}{\operatorname{span}} % SH: redefining this messes up the amsmath align environment
\newcommand{\lin}{\operatorname{lin}}
\newcommand{\cont}{\operatorname{cont}}
%\newcommand{\dom}{\operatorname{dom}}
\newcommand{\dto}{\downarrow}
\def\longto{\mathop{\longrightarrow}\limits}
\newcommand{\ninf}{\longto_{n\to\infty}}
%\newcommand{\prl}{^\parallel}
\newcommand{\prl}{^{/\!/}}
\newcommand{\prp}{^\perp}
\def\ipr{\iprod}
\newcommand{\icon}{\odot} %infimal convolution

\usepackage{bbm}
\renewcommand{\chr}{\boldsymbol{\mathbbm{1}}} % characteristic function
%\renewcommand{\pred}[1]{\chr_{\left\{ #1 \right\}}}
\renewcommand{\pred}[1]{\chr[ #1 ]}
\newcommand{\ind}{\mathbb{I}}
\newcommand{\hf}{{\ts\oo2}}

\newcommand{\rhs}{\operatorname{RHS}}
\newcommand{\lhs}{\operatorname{RHS}}

%\renewcommand{\phi}{\varphi}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\barx}{{\bar\x}}
\newcommand{\lam}{\lambda}
\newcommand{\blam}{\boldsymbol{\lam}}
\newcommand{\bblam}{\bar\blam}
\newcommand{\ze}{\vec0}
\renewcommand{\L}{\calL}

\renewcommand{\P}{\mathrm{(P)}}
\newcommand{\D}{\mathrm{(D)}}

\renewcommand{\a}{{\vec a}}
\newcommand{\x}{{\vec x}}
\newcommand{\y}{{\vec y}}
\newcommand{\z}{{\vec z}}
\renewcommand{\c}{{\vec c}}
\renewcommand{\u}{{\vec u}}
\renewcommand{\v}{{\vec v}}
\newcommand{\w}{{\vec w}}
\renewcommand{\b}{{\vec b}}
\newcommand{\g}{{\vec g}}
\newcommand{\p}{{\vec p}}
\renewcommand{\r}{{\vec r}}
\renewcommand{\d}{{\vec d}}
\newcommand{\bP}{{\vec P}}

\newcommand{\Note}{\noindent{\bf Note. }}
\newcommand{\Thm}{\noindent{\bf Thm. }}
\newcommand{\Claim}{\noindent{\bf Claim. }}
\newcommand{\Pf}{\noindent{\bf Proof. }}
\newcommand{\Lem}{\noindent{\bf Lemma. }}
\newcommand{\Def}{\noindent{\bf Definition. }}
\newcommand{\eq}{&=&}

\def\eps{\varepsilon}
\newcommand{\Rni}{\R_{{}^{{}_{\ge}}}} % non-increasing
\newcommand{\Rp}{\R_{+}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\renewcommand{\Z}{\mathcal{Z}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\Rcc}{[-\infty,+\infty]}
\newcommand{\Roo}{(-\infty,+\infty)}
\newcommand{\Rco}{[-\infty,+\infty)}
\newcommand{\Roc}{(-\infty,+\infty]}

\newcommand{\T}{\mathcal{T}}

%\renewcommand{\int}{\operatorname{int}}
\newcommand{\cl}{\operatorname{cl}}

\newcommand{\E}{\text{{\bf E}}}

\newcommand{\und}[1]{\underline{#1\mkern-4mu}\mkern4mu }
% short underline, like a ``downstairs bar''

%\newcommand{\tabline}{{\cline{1-3}}}
%\def\tabline{\\[-10pt]\cline{1-3}}
%\def\tabline{\\\hline}
%\newcommand{\tabline}{\\\midrule{1-3}}
\newcommand{\tabline}{\\--&-&-----\\}
%\newcommand{\tabline}{\\\cline{1-2}}


\newcommand{\comp}{\kappa}
\newcommand{\Comps}{\mathcal{K}}
\newcommand{\recon}{\rho}
\newcommand{\Recons}{\mathcal{R}}
\newcommand{\size}{k}
%\newcommand{\loss}{\ell}
%\newcommand{\sizefunc}{{\rm size}}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\Funcs}{\hat{\F}}
\renewcommand{\mod}{{\rm MOD}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\nats}{\mathbb{N}}
\newcommand{\nsamp}{n}
\newcommand{\Pz}{P}
\newcommand{\Rate}{{\cal E}}
\newcommand{\UC}{\Rate_{{\rm uc}}}
\newcommand{\AgRate}{\Rate_{{\rm ag}}}
\newcommand{\Log}{{\rm Log}}
\newcommand{\bpi}{\boldsymbol{\pi}}

\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}

%\newcommand{\hide}[1]{}

